Robust Visual Sim-to-Real Transfer for Robotic Manipulation

Learning visuomotor policies in simulation is much safer and cheaper than in the real world. However, due to discrepancies between the simulated and real data, simulator-trained policies often fail when transferred to real robots. One common approach to bridge the visual sim-to-real domain gap is domain randomization (DR). While previous work mainly evaluates DR for disembodied tasks, such as pose estimation and object detection, here we systematically explore visual domain randomization methods and benchmark them on a rich set of challenging robotic manipulation tasks. In particular, we propose an off-line proxy task of cube localization to select DR parameters for texture randomization, lighting randomization, variations of object colors and camera parameters. Notably, we demonstrate that DR parameters have similar impact on our off-line proxy task and on-line policies. We, hence, use off-line optimized DR parameters to train visuomotor policies in simulation and directly apply such policies to a real robot. Our approach achieves 93% success rate on average when tested on a diverse set of challenging manipulation tasks. Moreover, we evaluate the robustness of policies to visual variations in real scenes and show that our simulator-trained policies outperform policies learned using real but limited data. Code, simulation environment, real robot datasets and trained models are available at https://www.di.ens.fr/willow/research/robust_s2r/.

==> figures/experimental_setup.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{svg/experimental_setup.png}
  \caption{Experimental setup. The robotic platform comprises a robotic arm
    equipped with a robotiq's RG2 gripper. Camera 0 on the image (left side) and Camera
    1 (right side) are calibrated using the AprilTag on the center of our
    workspace \todo{update figure with a clean view, correct size, and add arrows to show where elements are located and the workspace area}.}
  \label{fig:experimental_setup}
\end{figure}

==> figures/rendering_comp.tex <==
\begin{figure}[t]
 \centering
 \includegraphics[width=\linewidth]{svg/rendering_comp.pdf}
 \caption{\textbf{Comparison between the three considered rendering qualities.} The main difference between scenes can be observed on each element boundaries where aliasing is produced. \todo{Remove the figure; put the results in table 2?}}
  \label{fig:rendering_comp}
\end{figure}

==> tables/policy_ablation.tex <==
\begin{table}[t]
\small
\vspace{0.2cm}
\setlength\tabcolsep{2.7pt}
\centering
\begin{tabular}{lcc}
  \toprule
  Model & Stacking (\%) & Sweeping (\%)\\
  \midrule
  Baseline & 39.6 & 32.8 \\
  + Multiple viewpoints & 61.6 & - \\
  + History & 96.4 & 80.0 \\
  + Proprioceptive info. & 100 & 98.0 \\
  \bottomrule
\end{tabular}
\caption{Model ablation.}
\label{table:policy_ablation}
\end{table}

==> tables/real_tasks_bis.tex <==
\begin{table*}
\centering
\tabcolsep=0.13cm
\begin{tabular}{cccccccccccccc} \toprule
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}img\\ aug\end{tabular}} & \multicolumn{2}{c}{Texture} & \multirow{2}{*}{Light} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Obj\\ color\end{tabular}} & \multirow{2}{*}{Camera} & \multicolumn{8}{c}{Success rate} \\
 & Proc & ACG &  &  &  & Stacking & Box-retrieving & Assembling & Pushing  & Pushing-to-pick & Sweeping & Rope-shaping & Average \\ \midrule 
 \checkmark & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0/20 & 0/20 & 0/20 & 0/20 & 0/20 & 0/20 & 0/20 & 0/20 \\ \midrule 
 \checkmark & $\times$ & \checkmark & $\times$ & $\times$ & $\times$ & 15/20 & 16/20 & 7/20 & 13/20 & 11/20 & 9/20 & 8/20 & 11.3/20 \\ \midrule 
 \checkmark & $\times$ & \checkmark & \checkmark & \checkmark & $\times$ & 17/20 & 15/20 & 13/20 & 18/20 & 13/20 & 11/20 & 11/20 & 14/20 \\ \midrule 
  \checkmark & $\times$ & \checkmark & \checkmark & \checkmark & \checkmark & 20/20 & 17/20 & 16/20 & 18/20 & 17/20 & 19/20 & 18/20 & 18.6/20 \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Performance for seven manipulation tasks trained in simulation and evaluated on a real robot.} We evaluate policies by running 20 episodes on the robot for each task and report the success rate (\%).}
\label{table:policy_success}  
\end{table*}


==> tables/rendering_quality.tex <==
\begin{table}[t]
\small
\setlength\tabcolsep{2.7pt}
\centering
\begin{tabular}{lcc}
  \toprule
  Rendering quality & Test error (cm) \\
  \midrule
  Low & 2.22 \\
  Medium & 1.96 \\
  High & \textbf{0.95} \\
  \bottomrule
\end{tabular}
\caption{Effects of rendering quality on sim2real transfer.}
\label{table:rendering_quality}
\end{table}

